Improved Static Analysis of Parameterised Boolean Equation Systems using Control Flow Reconstruction

We present a sound static analysis technique for fighting the combinatorial explosion of parameterised Boolean equation systems (PBESs). These essentially are systems of mutually recursive fixed point equations ranging over first-order logic formulae. Our method detects parameters that are not live by analysing a control flow graph of a PBES, and it subsequently eliminates such parameters. We show that a naive approach to constructing a control flow graph, needed for the analysis, may suffer from an exponential blow-up, and we define an approximate analysis that avoids this problem. The effectiveness of our techniques is evaluated using a number of case studies.

==> macros.tex <==
\usepackage{mathtools}
\usepackage{ifthen}

\makeatletter
\def\slashedarrowfill@#1#2#3#4#5{%
  $\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
   \relax#5#1\mkern-7mu%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mathclap{#3}\mathclap{#2}%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mkern-7mu#4$%
}
\def\rightslashedarrowfill@{%
  \slashedarrowfill@\relbar\relbar{\raisebox{.12em}{\tiny/}}\rightarrow}
\newcommand\xslashedrightarrow[2][]{%
  \ext@arrow 0055{\rightslashedarrowfill@}{#1}{#2}}

\newcommand{\JK}[1]{\marginpar{{\color{red}{#1}}}}
\newcommand{\TW}[1]{\marginpar{{\color{red}{#1}}}}
\newcommand{\comment}[1]{}

\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\etc}{\emph{etc.}\xspace}
\newcommand{\viz}{\emph{viz.}\xspace}
\newcommand{\ibid}{\emph{ibid.}\xspace}
\newcommand{\etal}{\emph{et al.}\xspace}

% Data types
\newcommand{\B}{\ensuremath{\mathbb{B}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}

\newcommand{\transition}[1]{\ensuremath{\stackrel{a}{\to}}}
\newcommand{\cfp}[1]{\ensuremath{{#1}^{\mathit{CFP}}}}
\newcommand{\dap}[1]{\ensuremath{{#1}^{\mathit{DP}}}}
\newcommand{\getcfp}[1]{\ensuremath{\mathit{CFP}(#1)}}
\newcommand{\getdap}[1]{\ensuremath{\mathit{DP}(#1)}}
\newcommand{\type}[1]{\ensuremath{\mathcal{T}(#1)}}
\newcommand{\updatestate}[3]{\ensuremath{{#1}[#2 \mapsto #3]}}
\newcommand{\bisim}{\ensuremath{\leftrightarroweq}}
\newcommand{\free}[1]{\ensuremath{\mathit{FV}(#1)}}

\newcommand{\isdef}{\ensuremath{=}}

\newcommand{\dataname}{\mathsf{arg}}
\newcommand{\predname}{\mathsf{pv}}
\newcommand{\predinstname}{\mathsf{PVI}}
%\newcommand{\dataphi}[2]{\dataname(#1, #2)}
\newcommand{\dataphi}[3][]{\ifthenelse{\equal{#1}{}}{\dataname(#2, 
#3)}{\dataname_{#1}(#2, #3)}}
\newcommand{\predphi}[2]{\predname(#1, #2)}
\newcommand{\predinstphi}[2]{\predinstname(#1, #2)}
%\newcommand{\predinst}[1]{\predinstname(#1)}
%\newcommand{\data}[1]{\dataname(#1)}
%\newcommand{\pred}[1]{\predname(#1)}
\newcommand{\npred}[1]{\mathsf{npred}(#1)}
\newcommand{\PBES}{\ensuremath{\mathcal{E}}}
\newcommand{\emptyPBES}{\ensuremath{\emptyset}}
\newcommand{\dataenv}{\ensuremath{\delta}}
\newcommand{\predenv}{\ensuremath{\eta}}
\newcommand{\sem}[3]{\ensuremath{\llbracket#1\rrbracket#2#3}}
\newcommand{\semset}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\varset}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\sort}[1]{#1}
\newcommand{\subst}[2]{\ensuremath{#2 / #1}}
\newcommand{\true}{\ensuremath{\mathit{true}}}
\newcommand{\false}{\ensuremath{\mathit{false}}}
\newcommand{\quantifier}{\ensuremath{\mathsf{Q}}}
\newcommand{\depends}[2]{\ensuremath{\mathsf{Dep}(#1,#2)}}
\newcommand{\relevant}[2]{\ensuremath{\mathsf{Rel}_{{#1}}(#2)}}
\newcommand{\relevantCFG}[2]{\ensuremath{\mathsf{Rel}^{\mathit{CFG}}_{{#1}}(#2)}}
\newcommand{\relevantLocCFG}[2]{\ensuremath{\mathsf{Rel}^{\mathit{CFG-loc}}_{{#1}}(#2)}}
\newcommand{\cfl}[1]{\ensuremath{\mathsf{CFL}(#1)}}
\newcommand{\resetname}{\ensuremath{\mathsf{Reset}}}
\newcommand{\reset}[2]{\ensuremath{\resetname_{{#1}}(#2)}}
\newcommand{\resetvars}[3]{\ensuremath{\resetname^{{#1}}_{{#2}}({#3})}}
\newcommand{\init}[1]{\ensuremath{\mathsf{init}(#1)}}
\newcommand{\rules}[2]{\ensuremath{\mathsf{rules}_{#1}(#2)}}
\newcommand{\changed}[1]{\ensuremath{\bar{#1}}}
\newcommand{\consistent}{\ensuremath{\doteqdot}}
\newcommand{\correnv}[1]{\ensuremath{\Theta_{#1}}}
\newcommand{\signature}[1]{\ensuremath{\mathsf{sgt}(#1)}}
\newcommand{\block}[2]{{#2\rceil{#1}}}
\newcommand{\bnd}[1]{\ensuremath{\mathsf{bnd}(#1)}}
\newcommand{\dep}[1]{\ensuremath{\mathsf{dep}(#1)}}
\newcommand{\rhs}[1]{\ensuremath{\varphi_{#1}}}

\newcommand{\semantic}{\mathit{sem}}
%\newcommand{\syntactic}{\mathit{syn}}
\newcommand{\syntactic}{}
\newcommand{\local}{\mathit{l}}
\newcommand{\localtoglobal}{\mathit{gloc}}

%\newcommand{\ind}[2]{\ensuremath{{#1}[{#2}]}}
\newcommand{\ind}[2]{\ensuremath{#1_{#2}}}
\newcommand{\var}[2][]{\ifthenelse{\equal{#1}{}}{\vec{#2}}{\ind{\vec{#2}}{#1}}}
\newcommand{\val}[2][]{\ifthenelse{\equal{#1}{}}{\vec{#2}}{\ind{\vec{#2}}{#1}}}
\newcommand{\semval}[2][]{\ifthenelse{\equal{#1}{}}{\sem{\vec{#2}}{}{}}{\sem{\ind{\vec{#2}}{#1}}}{}{}}

\newcommand{\Q}{\ensuremath{\mathsf{Q}}}
\newcommand{\sourcename}{\ensuremath{\mathsf{source}}\xspace}
\newcommand{\source}[3]{\sourcename(#1, #2, #3)}
\newcommand{\destname}{\ensuremath{\mathsf{target}}\xspace}
\newcommand{\dest}[3]{\destname(#1, #2, #3)}
\newcommand{\copiedname}{\ensuremath{\mathsf{copy}}\xspace}
\newcommand{\copied}[3]{\copiedname(#1, #2, #3)}
\newcommand{\valuesname}{\ensuremath{\mathsf{values}}}
\newcommand{\values}[1]{\ensuremath{\valuesname(#1)}}
\newcommand{\len}[1]{\ensuremath{\mathit{len}(#1)}}
\newcommand{\occname}{\ensuremath{\mathsf{occ}}}
\newcommand{\paramname}{\ensuremath{\mathsf{par}}}
\newcommand{\occ}[1]{\ensuremath{\occname(#1)}}
\newcommand{\param}[1]{\ensuremath{\paramname(#1)}}
\newcommand{\conjunct}[2]{\ensuremath{#1,#2}}
\newcommand{\disjunct}[3]{\ensuremath{#1,#2,#3}}
\newcommand{\CFL}{\ensuremath{\mathit{CFL}}}
\newcommand{\VCFG}{V^{\semantic}}
\newcommand{\VCFGsyn}{V^{\syntactic}}
\newcommand{\VCFGloc}{V^{\local}}
\newcommand{\ECFG}{\xrightarrow{\semantic}}
\newcommand{\ECFGsyn}[1][]{\xrightarrow[\syntactic]{#1}}
%\newcommand{\ECFGloc}[1]{\xrightarrow[\local]{#1}}
\newcommand{\ECFGloc}[1][]{\xhookrightarrow{#1}}
\newcommand{\nECFG}{\xslashedrightarrow{\semantic}{}}
\newcommand{\nECFGsyn}[1]{\xslashedrightarrow[#1]{\syntactic}}
\newcommand{\nECFGloc}[1]{\xslashedrightarrow[#1]{\local}}

\newcommand{\cardinality}[1]{|#1|}

\newcommand{\rel}[1]{\ensuremath{\mathrel{#1}}}
\newcommand{\R}[1]{R^{#1}}

\newcommand{\markingname}{L}
\newcommand{\markingsn}[2]{\markingname_{#1}^{#2}}
\newcommand{\marking}[2]{#1(#2)}
\newcommand{\markrel}[1]{\R{#1}}
\newcommand{\guardname}{\mathsf{guard}}
\newcommand{\guard}[2]{\guardname^{#1}(#2)}
\newcommand{\guardedname}{\mathsf{guarded}}
\newcommand{\guarded}[1]{\mathsf{guarded}{(#1)}}
\newcommand{\simpleguardname}{\mathsf{sguard}}
\newcommand{\simpleguard}[2]{\simpleguardname(#1, #2)}
\newcommand{\significantname}{\mathsf{sig}}
\newcommand{\significant}[1]{\significantname(#1)}
\newcommand{\fp}[2]{\mathsf{FP}^{#1}(#2)}
\newcommand{\fpguard}[2]{\mathsf{FP}^{#1}_{#2}}
\newcommand{\fpsimple}[2]{\mathsf{FP}^{#1}_{s}(#2)}
\newcommand{\CFP}{\mathit{CFP}}
\newcommand{\DP}{\mathit{DP}}
\newcommand{\belongsto}[1]{\mathsf{belongs}(#1)}
%\newcommand{\affects}[2]{#1~\mathsf{affects}~#2}
\newcommand{\affects}[2]{#1 \in \free{#2}}
\newcommand{\simplifyname}{\mathsf{simplify}}
\newcommand{\simplify}[1]{\simplifyname(#1)}

\newcommand{\mcrlKw}[1]{\mathbf{#1}}
\newcommand{\mcrlAct}[1]{\mathit{#1}}

